Support Generation for Robot-Assisted 3D Printing with Curved Layers

Robot-assisted 3D printing has drawn a lot of attention by its capability to fabricate curved layers that are optimized according to different objectives. However, the support generation algorithm based on a fixed printing direction for planar layers cannot be directly applied for curved layers as the orientation of material accumulation is dynamically varied. In this paper, we propose a skeleton-based support generation method for robot-assisted 3D printing with curved layers. The support is represented as an implicit solid so that the problems of numerical robustness can be effectively avoided. The effectiveness of our algorithm is verified on a dual-material printing platform that consists of a robotic arm and a newly designed dual-material extruder. Experiments have been successfully conducted on our system to fabricate a variety of freeform models.

==> text/algorithm.tex <==
\section{Algorithms for support tree generation}\label{secAlgorithm}

The input of our algorithm is the tetrahedron mesh $\mathcal{T}^m$ of the given model and the vector field $\mathbf{V}(\mathbf{x})$ guiding the accumulation process of printing. The $\mathbf{V}(\mathbf{x})$ is naturally provided to guide the generation of curved layers in \cite{Fang_SIG20}. For other cases (e.g.\cite{Etienne_SIG19}), it is straightforward to calculate $\mathbf{V}(\mathbf{x})$ from the height field $z(\nabla h_t)$  of model, which could be described as scalar field $\mathbf{G}(\mathbf{x})$, by using piece-wise linear function: 
\begin{align}
\mathbf{V}(\mathbf{x}) = \nabla \mathbf{G}(\mathbf{x}) = \left( \sum_{i=1}^4 a_i g_i,  \sum_{i=1}^4 b_i g_i,  \sum_{i=1}^4 c_i g_i \right)
\end{align}
where $(a_i,b_i,c_i)$ being the $x$-, $y$- and $z$-components of the vector $(\mathbf{p}_{i+1} - \mathbf{p}_{i+3}) \times (\mathbf{p}_{i+1} - \mathbf{p}_{i+2}) / 6 v_e$. Note that, the index $i$ of $\mathbf{p}_i$ is recycled in the above formula, and the $v_e$ means the volume of tetrahedron element $e$ which is defined by its four nodes $\{\mathbf{p}_i\}_{i=1,\cdots,4}$. In short, the gradient $\nabla G(\mathbf{x})$ is in a simple form as the linear combination of the field values $\{g_i\}$ on the four nodes, and it describes the trend of the scalar field growth. 

The direction of $\mathbf{V}(\mathbf{x})$ is the local printing direction $d_p$ installed at the center of the tetrahedron elements, the criteria of overhang face $\mathcal{F}_o$ is defined as \cite{Hu_CAD15}
\begin{equation}\label{overhang detection}
    n_f \cdot d_p + \sin(\alpha) \leq 0
\end{equation}
where $n_f$ means the normal of the boundary face of tetrahedron mesh $\mathcal{T}^m$ and so $\mathcal{F}_o$ is defined on the boundary of $\mathcal{T}^m$. Specifically, self-support is achieved when the $d_p$ falls into the cone determined by $n_f$ and self-support angle $\alpha$, which depends on the printing materials, temperature, and nozzle size, so it should be determined according to the real printing situation.

For fabrication requirements like strength reinforcement and surface quality improvement, the support structure is needed in most cases. Even though the support-free requirement is satisfied in many models. The support generation method is still a valuable strategy for complementing curved layer printing. we proposed an implicit-surface-based tree support generation method for curved layer printing. The specific steps shown below:
\begin{itemize}
  \item Initial guess of support envelop hull of model and compatible curved layers generation;
  \item Tree-like support skeleton tracing;
  \item Generation of the implicit surface of tree-skeleton;
  \item Boolean operation between implicit surface and compatible layers, and contour toolpath generation;
\end{itemize}

\subsection{Initial guess of support envelop and the compatible layers generation}

There is a straightforward assumption that curved slicing could be supported completely if the support structure surrounds the entire model. After collecting the nodes from overhang faces $\mathcal{F}_o$, line segments grow from overhang nodes and decent toward the bottom along the inverse direction of local printing direction $-d_p$. In order to avoid the intersection of the line segment with the bottom plane very far from the origin, when $-d_p$ is almost parallel to the bottom plane, we introduce two variables: rotation angle and step size, and use polyline to gradually approach the bottom plate. When the direction of the polyline is already straight downward, we will keep the decent direction as (0, 0, -1). The polyline nodes and all the surface nodes of tetrahedron mesh will be mixed to generate a convex hull $\mathcal{C}$. The parameters of decent angle and length are obtained from users.

%\tianyu{Here we need a figure to show the initial envelope and compatible layers generation.}

Then the envelope tetrahedron mesh $\mathcal{T}^c$ built from $\mathcal{C}$ is used to obtain the compatible layers including model material and support material layers. In specifically, model layers comes from $\mathcal{T}^m$ and the compatible support layers are obtained from $\mathcal{T}^s = \mathcal{T}^c - \mathcal{T}^m$. $\mathcal{T}^s$ and $\mathcal{T}^m$ share the same scalar field and vector field at the contact boundary, therefore, the boundary of two compatible layers (one support layer and one model layer) share the same nodes and edges.

Here all input data are listed to facilitate further illustration of the algorithm below:
\begin{itemize}
    \item Compatible layer sequence $\{\mathcal{L}^c_i\} = \{\mathcal{L}^m_i \cap \mathcal{L}^s_i\}$;
    \item Support-free angle $\alpha$ which is given by users.
    \item Tetrahedron mesh $\mathcal{T}^m$ and its vector field $\mathbf{V}(\mathbf{x})$, which serve as printing direction
\end{itemize}

\subsection{Generation of tree-like support skeleton}
All the overhang nodes on the surface of model mesh $\mathcal{T}^m$ are copied as origin nodes $\{\mathcal{P}^s_o\}$ of the support tree. A set of rays are built from each $\{P^s_o\}$ along the inverse direction of the vector field $-d_p$ to intersect with the first bellow curved layer. It should be emphasized that the overhang nodes are transferred from the model surface onto the curved layers %\tianyu{key statement}. 
And then the tree tracing and merging will be iteratively conducted at the rest below layers $\{\overline{\mathcal{L}}^c_i\}$.

Each face of compatible layers may own more than one intersection node or zero. To clearly explain the tracing and merging method, a planar illustration is shown in Fig.\ref{fig:branch_tracing}. There are three intersection nodes on the $\mathcal{F}^s_j$ of the layer $\mathcal{L}^s_i$. The n-ring neighbour of $\mathcal{F}^s_j$ is defined as $\mathcal{O}^s_j$ and there are another three intersection nodes on the $\mathcal{O}^s_j$. 
%\tianyu{We maybe need a pseudo-code here.}

Firstly, the host node is defined as who owns the greatest number of tree branches and is projected directly along the inverse growing direction which is decided by the face normal of $\mathcal{F}^s_j$. The host node $\mathcal{P}^s_h$ is marked as the red one and the red arrow means the projection process of the host node. \tianyu{It should be noted that when all nodes have the same degree, we randomly select a host node.} Next, the intersection nodes in $\mathcal{F}^s_j$ and $\mathcal{O}^s_j$ are treated as follower nodes $\mathcal{P}^s_f$, and the branches growing from them are rotated towards the new intersection node of the host node $\mathcal{P'}^s_h$. In Fig.\ref{fig:branch_tracing}, the following nodes marked with “2” and “5” shoot green arrows toward the below layer $\mathcal{L}^s_{i-1}$. However, the support tree itself should be support-free, in other words, the support tree should support itself before supporting models. This requirement is translated as the rotation angles of arrows should be less than $\alpha$,  where $\alpha$ is the self-support angle. Hence, rotation arrows should not be out of the orange cone in Fig.\ref{fig:branch_tracing}. The arrow rotates with the maximum allowed angle and intersects with $\mathcal{L}^s_{i-1}$ at node “$5'$”,  while the arrow starting from intersection node “2” can directly point to “$1'$” in the layer $\mathcal{L}^s_{i-1}$ and the endpoint of arrows shot both from host node “1” and following node “2” are merged into “$1'$”. And the branch number of node “2” are absorbed by “$1'$”. The size of ring neighbour means how many rings of neighbour faces are collected for the host node and the default value of rings is 3 in our system. Each branch whose start node is on the layer $\mathcal{L}^s_i$ and the end node is on the layer $\mathcal{L}^s_{i-1}$ is constructed as an edge into a tree mesh. The iteration of tracing will be stopped when the nodes hit on the platform or model layers.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fig/branch_tracing.jpg}
\put(-240,2){\small \color{black}(a)}
\put(-90,2){\small \color{black}(b)}
\put(-115,38){\small \color{black}$\mathcal{L}^s_{i}$}
\put(-115,10){\small \color{black}$\mathcal{L}^s_{i-1}$}
\caption{(a) Illustration of tree branch tracing and merging. “A-A” means the cross-section of $\mathcal{L}^s_{i}$, red node is the host node and green nodes are the following nodes and nodes with the symbol prime are the intersection node of tree branches on the next layer $\mathcal{L}^s_{i-1}$. Notes that all the operation is conducted on the curved layers. (b) In the tree skeleton after tracing, the red facets mean the overhang regions.}
  \label{fig:branch_tracing}
\end{figure}

\subsection{Construction of implicit surface of tree skeleton}

The edge-based implicit surface is built from the tree skeleton, and it is used to cut the curved layers $\{\mathcal{L}^s_i\}$ of support material generated from the enveloped tetrahedron mesh $\mathcal{T}^c$. After that, the Boolean operation is conducted between layer mesh and implicit surface, so it is robust and time-saving compared to the Boolean operation between meshes.

The support tree $\Omega$ is represented as a mesh with interconnected tree skeletons, which is stored as $\Omega=(\mathcal{V},\mathcal{E})$ with a set of nodes and a set of branches or edges. Each $v_i\in\mathcal{V}$ defines the position of nodes, and each edge $e_j\in\mathcal{E}$ is represented as a pair of vertices associated with the radius of the edge’s corresponding strut as $e_j=(v_s,v_e,r_j)$. The support tree is represented as an implicit surface defined around the tree skeleton and its corresponding surface is formulated as
\begin{equation}
\mathcal{S}(\Omega)=\{\mathbf{p} | F (\mathbf{p}) = 0 (\forall \mathbf{p} \in\mathbf{R}^\mathbf{3})\},
\end{equation}
where $F(\cdot)$ is an implicit distance value between query point $\mathbf{p}$ and tree skeleton $\Omega$, it can be realized by convolution surface. Here we just show the simplified equation and concept, more details could be found at \cite{Liu_21JCISE}.
%\begin{equation}\label{implicit solid equation}
%F(\mathbf{p})=-C+(f\otimes h)(\mathbf{p}),
%\end{equation}
%with $h:\mathbf{R}^\mathbf{3}\rightarrow\mathbf{R}$ is a geometric function representing the skeleton $\Omega$ and $C$ is a constant iso-value defined according to the radii defined on the skeleton edges. The quartic polynomial kernel function is adopted, then the function $F(\cdot)$ could be written into the edge form as
\begin{equation}
F(\mathbf{p})=-C+ \sum_{e_j \in \Omega} r_i \int_{\mathbf{x} \in e_j } f(\mathbf{p}-\mathbf{x}) d e_j
\label{implicit solid equation}
\end{equation}
where $C$ is a constant iso-value defined according to the radii defined on the skeleton edges and the quartic polynomial kernel function is adopted. % The convolution integral along an edge can be computed by an analytical close-from and then 
The field value at point $\mathbf{p}$ contributed by $e_j$ can be computed as
\begin{equation}
\begin{aligned}
    F_{e_j} (\mathbf{p}) &= r_j \int_{s_1}^{s_2} (1-\frac{\| \mathbf{p}-\mathbf{x(s)} \|^2}{R^2})ds\\&= \frac{r_j}{15R^4} (3l^4 s^5-15al^2 s^4+20a^2 s^3 )\|_{s_1}^{s_2}
\end{aligned}
\end{equation}
where $R$ being the support-size, $l=\|\mathbf{p}_2- \mathbf{p}_1\|$ and $a=(\mathbf{v}_s-\mathbf{p}_1)\cdot(\mathbf{p}_2 -\mathbf{p}_1)$. When the iso-value $C$ in Eq.(\ref{implicit solid equation}) is fixed, we can adjust the value of $r_j$ to change the radius of tree branches generated from each skeleton edge $e_j$. \tianyu{add more explanation here.} Such as decreasing the value of $r_j$, the point with the same iso-value will be closer to $e_j$ thus reducing the branch radius. In our formulation, the support size of each kernel function is not changed when using different values of $e_j$s for different branches. And the radius of each $r_j$ is decided by the branch number which is recorded during the tree skeleton building. Inspired by the trees in the natural environment, there is a straightforward idea that the cross-section area of all branches should be equal to the area of the trunk, whose radius is $r$.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fig/implicit_surface.jpg}
\put(-240,6){\small \color{black}(a)}
\put(-160,6){\small \color{black}(b)}
\vspace{-5pt}
\caption{The comparison of implicit surface of tree-support structure building by Marching Cube (MC) with (a) fixed branch radius; (b) dynamic branch radius. The latter one is becoming gradually thicker from the top of the tree to the trunk.}
\label{fig:implicit_surface}
\end{figure}

\begin{equation}
    \pi r^2 = \sum^m_{k = 1} \pi r_k^2
\end{equation}
where the $m$ is the number of branches. This calculation method of branch radius could obtain a support tree with thick trunks and slim branches as Fig.\ref{fig:implicit_surface}(b) shows. \tianyu{However, the truck part of  Fig.\ref{fig:implicit_surface}(a) is too slim to support the model itself.}

\subsection{Boolean operation and contour toolpath generation}
In this section, the Boolean operation between support layers $\{\mathcal{L}^s_i\}$ and implicit surface $\mathcal{S}(\Omega)$ is conducted and obtain the final slimmed support layers $\{\mathcal{L'}^s_i\}$. The topology relationship of faces is shown in Fig.~\ref{fig:tree_support_extraction}(a), $v_i (i = 0,1,2)$ means each node of triangle and $e_i (i = 0,1,2)$ is represented by node pairs. Each node of support layers serves as a query node and we calculate its implicit distance, there are four cases:
\begin{itemize}
    \item $\forall{F(v_i) > 0}$: Implicit distance value of three nodes of face $f_i$ are all larger than zero, then $f_i$ is kept.
    \item $\forall{F(v_i) \leq 0}$: Implicit distance value of three nodes is all less than zero, then this facet will be discarded from slimmed support layers.
    \item If the distance value of only one node is larger than zero while the other two nodes are not, iso-surface $F(\cdot)= 0$ will cut this facet and keep the small triangle formed by two intersection nodes and the original node. (See the marker 1 in Fig.\ref{fig:tree_support_extraction}).
    \item If the distance value of two nodes is larger than zero while only one node is not, $F(\cdot)= 0$ will pass through this facet and collect the quadrilateral part of it. Furthermore, the quadrilateral is split into two triangles, shown as marker 2 in Fig.\ref{fig:tree_support_extraction}).
\end{itemize}

In the final stage, contour toolpath %\tianyu{add more in figure 6}
is generated for slimmed support layers and original model layers. After that, the tree-supported printing path has been generated, and the experimental verification is completed on our system.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fig/tree_support_extraction.jpg}
\put(-243,5){\small \color{black}(a)}
\put(-156,5){\small \color{black}(b)}
\put(-75,5){\small \color{black}(c)}
\caption{Illustration of slime tree support generation. (a) Cases when conducting trimming operation; (b) The compatible layers (support layer and model layer); (c) The rest support layer after Boolean operation and original model layer.
%\tianyu{Figure will be updated considering curved boundary of implicit surface, remove p0 p1 p2}
}
\label{fig:tree_support_extraction}
\end{figure}

==> text/conclusion.tex <==
\section{Conclusion and Discussion}\label{secConclusion}
We build a dual-extruder robot printing system to fabricate support for curved layers. The 6-DOF motion will drive the extrusion tool to achieve the multi-axis printing, meanwhile, the platform is fixed and the PLA and PVA are used to print the model and support layers. The core part of our system is an algorithm to obtain tree support for given curved slices which could follow the strength-reinforcement or surface quality improvement requirements. The tree structure could decrease the support volume and printing time and also implicit surface-based Boolean method could get a robust performance. Our experimental tests give promising results, and the models with large overhangs can be fabricated with well support structure. 
There are still some limitations in our current implementation of the support generation method, which fall into the following aspects. 

%1. only support out-support;
%2. many jump;
%3. rotation case;
%4. filed-based method (generate a field for it)

\vspace{3pt}\noindent 1) \textit{Outside support}: Our method only generates the tree support for the outside boundary of the model, not the inner, so it is not suitable for hollowed models . Our models are printed in solid, which is reasonable for the strength-reinforcement cases where the anisotropic property is borrowed to increase the mechanical strength of the model \cite{Fang_SIG20}.

\vspace{3pt}\noindent 2) \textit{Jump}: The support patches are trimmed as some separated regions, which will bring repeatedly retraction operation when jumping among these regions, and then decrease the printing quality. We control the direction of tree tracing towards the center of the platform to decrease the number of separated regions.

\vspace{3pt}\noindent 3) \textit{Input}: Our algorithm needs the growing field of the model as input data, so it is needed to transfer the results of other papers' methods into the vector field.

%\vspace{3pt}\noindent 4) \textit{Table rotation}: The static and dynamic stability of the model during the printing process is not considered.

\vspace{3pt}\noindent In summary, although our robot-assisted additive manufacturing platform gives promising results in experiments, there are still a few challenges to be tackled in our future research.

==> text/intro.tex <==
\section{Introduction}\label{secIntro}

\textit{Similar} to the trend of subtractive machining from 3-axis to multi-axis, more and more attention has been paid to multi-axis additive manufacturing with the gradual maturity of flat printing. A large amount of its innovation has emerged in scientific research and further applied to industry fields, such as laying carbon fibre along the stress direction for aircraft wings, improving surface quality by moving nozzles along the curved working surface, etc. These applications and studies take advantage of the additional degrees of freedom (DOFs) from multi-axis 3D printing and the resulting benefits such as reduced support, enhanced strength, and improved surface quality. However, the support structure is impossible to avoid completely, especially, if the users would like to take advantage of the anisotropic of the filament to strength reinforcement (e.g., \cite{Fang_SIG20}).

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fig/teaser.jpg}
\put(-243,5){\small \color{black}(a)}
\put(-128,78){\small \color{black}(b)}
\put(-128,5){\small \color{black}(c)}
\put(-62,5){\small \color{black}(d)}
\caption{The robotic-assisted printing system and fabrication results. (a) UR5e robot arm associated with a dual-material extruder; (b) Support tree skeleton of model Yoga which is under strength reinforcement requirement; (c) The printing result of \cite{Fang_SIG20}; And (d) shows our printing results whose support volume is dramatically decreased than before.}
\label{figTeaser}
\end{figure}

\subsection{Motivation}
The robot arm has been widely used in the 3d printing field\cite{Bhatt_ADDMA20_survey, Urhal_19RCIM}. In the commercial 3D printing system, support generation is an essential component in the slicing engines, which greatly improves the versatility of slicing software. Although there are lots of algorithms developed to generate curved layers for multi-axis printing, fewer methods are proposed to generate support structures for curved layers. Our system uses a robotic arm to provide 6-DOF motion on the printing head, accompanied by a 2IN1 extruder system which can provide double filaments, one is for the model, and one is for support printing. Double filaments pass through one nozzle alternatively, hence the precision of printing is improved and simplifies the calibration steps compared to the strategy of changing the filament by converting nozzles.

Besides the hardware system, it is critical to efficiently and effectively generate curved layers to utilize the benefits of multiple axes. There has been a lot of pioneering work to decompose the model and generate a series of working surfaces. The anisotropic property of FDM\cite{Fang_SIG20} is used to improve the mechanical property of models. During the fabrication enabling step, support generation is conducted to realize the experimental verification. Although \cite{Dai_SIG18} could handle variable models for support-free requirements, the support generation method of curved layers is also necessary, as it can further broaden the generality of multi-axis curved layer printing and also the support is almost inevitable for strength reinforcement cases and surface quality improvement case. Hence the motivation of this work is to generate the tree-like support layers and toolpath for multi-axis vector printing. The most challenging issue is how to obtain a support layer set which is compatible with model layers, self-support and slimmed as tree shape. Fig.~\ref{figTeaser} shows the tree structure of a freeform model -- Yoga and its fabrication results. Note that, although FDM-based 3D printing is practised in our implementation, this method can also be applied to other types of AM e.g. CNC-based printing machines.

%\tianyu{!!! Why the curved support generation is hard to conduct???}

\begin{figure}[t]
\centering 
\includegraphics[width=\linewidth]{fig/hardware.jpg}
%\put(-240,80){\small \color{black}(a)}
%\put(-150,80){\small \color{black}(b)}
%\put(-70,80){\small \color{black}(c)}
%\put(-240,0){\small \color{black}(d)}
\caption{The hardware of the 3d printing system for FDM-based dual-material fabrication. A 2IN1 structure is installed onto the robot arm, different filaments pass through the Y-shaped tunnel alternatively. And the router is the core of communication between each controller (UR5e controller, Duet3D and PC).}
\label{figSysHardware}
\end{figure}

\begin{figure*}[t]
\centering 
\includegraphics[width=\linewidth]{fig/pipeline.jpg}
\put(-505,0){\small \color{black}(a)}
\put(-410,0){\small \color{black}(b)}
\put(-295,0){\small \color{black}(c)}
\put(-200,0){\small \color{black}(d)}
\put(-95,0){\small \color{black}(e)}
\put(-490,15){\small \color{black}$\mathcal{C}$}
\put(-505,103){\small \color{black}$\mathcal{T}^m$}
\put(-413,100){\small \color{black}$\{\mathcal{L}^m_i$\} }
\put(-355,15){\small \color{black}$\{\mathcal{L}^s_i\}$}
\put(-250,15){\normalsize \color{black}$\Omega$}
\put(-128,15){\small \color{black}$\mathcal{S}(\Omega)$}
\put(-78,15){\small \color{black}$\{\mathcal{L'}^s_i\}$}
\caption{Diagram to show the pipeline of tree support generation of curved layer printing. (a) Support envelop hull; (b) Compatible layer set; (c) Support tree skeleton; (d) Implicit surface of tree skeleton; (e) Slimmed support layers and model layers.}\label{fig:sys_pipeline}
\end{figure*}

\subsection{Related work}
Traditional 3D printing is widely used in lots of fields such as metal printing of turbo in aerospace \cite{Vafadar_AS21}, tooth aligner treatments in the medical field \cite{Sangeeth_POLYMERS21} and lattice structures shoes printing in sportswear \cite{Vanderploeg_IJFDTE17}. They are limited to three-axis movement with step motion along the Z axis. This kind of 2.5D printing method is easy to apply, robust in printing and popular on the customer side. However, low mechanical strength between layers, stair-case and large support requirement issues are frequently mentioned, Wulle et al.\cite{Wulle_CIRP17} analysed these types of limitations of the current 3D printing method and proposed that multi-axis AM enables completely new design possibilities going beyond current optimization and design strategies of conventional AM workpieces. Growing research work focuses on multi-axis printing. 

Robot-assisted printing platforms could provide extra DOFs, larger working space and could be built swiftly. Papers\cite{Dai_SIG18, Li_CAD21} built multi-axis FDM printers for support-less or even support-free printing, which is composed of a 6DOF robot arm (UR) and a fixed filament extruder. The robot holds the platform and workpiece to realize desirable posture with respect to the nozzle, meanwhile, filaments are synchronously controlled. Different from the above configuration, Soler et al. \cite{Soler_ACADIA17} reoriented the end-effector while the object remains fixed, which is suitable for fabricating bigger parts. Two robot arms are arranged to form the whole system \cite{Bhatt_ADDMA20} where 3 DOFs build-platform and a 3 DOFs extrusion tool are used to build thin shell parts. The decoupling of space translation and gesture control simplifies motion control. Ding et al. \cite{Ding_RCIM17} developed a robot-controlled system that couples a 6-axis robot arm with an additional 2-axis tilt and rotatory positioning systems. The redundant degree of freedom from the positioner can decrease the large space movement of the robot arm, and then the line speed of the tooltip will be even and the printing quality can also be improved. A similar configuration is also shown in \cite{Fang_SIG20}, this paper aims to utilize the anisotropic property of filament to reinforce the mechanical strength of the printed part. What's more, it provides a $\alpha$-hull based support generation method for overhang\cite{Evans_BOOK12} regions during the curved layer printing. More research on robotic additive manufacturing can be found in this extensive literature review \cite{Bhatt_ADDMA20_survey}.

In order to print the model with overhang regions, Vaissier et al. \cite{Vaissier_CAD19} firstly used a lattice cell to fill the support space as an initial guess, and then removed unnecessary lattice beams to obtain a tree-like support structure. Paper \cite{Dumas_SIG14} took advantage of the ability to bridge the gap of FDM and proposed a scaffold structure, which was composed of bridges and vertical pillars to support the overhang regions. This method could provide more stable support for printing compared with tree support. The self-support cone is used to decrease the usage of support material in \cite{Schmidt_SIG14}. A new type of tree-support, named Escaping Tree-Support (ET-Sup) is proposed to try to build all the supports onto the build plate to minimize the number of contact points \cite{Kwok_RPJ21}.  

However, these existing works only focus on the support generation for planar layer printing, less work is conducted for curved layer supporting structures.

\subsection{Contribution}

The major contribution of this paper is a tree-support generation approach for curved layer fabrication and the system for realizing multi-axis dual-material FDM on a robot-assisted system, which can be summarized as follows:
\begin{itemize}
    %\item Slimmer support generation considering self-support angle – less support, shorter printing time;
    %\item Generating support skeleton layer by layer considering the self-support property of printing – stable support;
    %\item Trimming based on implicit surface brings robust Boolean result;
    \item Construction of the robotic-assisted printing system with dual-extrusion mechanism;
    \item Development of effective tree support for curved layer printing based on the implicit surface function which highly reduces the usage of support material;
\end{itemize}
We use the specially designed G code to control the UR5e to print the model and slimmed support structure which is represented as a set of waypoints.

==> text/result.tex <==
\section{Implementation Details and Results}\label{secResult}

The tree support generation algorithm presented above has been implemented in a C++ program to generate slimmed support structure for multi-axis printing. The numerical library Eigen \cite{eigenweb} is employed as the solver of linear equations. The growing field $\mathbf{V}(\mathbf{x})$ of the given model $\mathcal{T}^m$ is used to guide the compatible layers $\{\mathcal{L}^c_i\}$ generation and overhang region detection. Tree-skeleton is traced from compatible support layers $\{\mathcal{L}^m_i\}$ and then used to generate an implicit surface to cut $\{\mathcal{L}^s_i\}$. The toolpath with contour pattern is generated and drives the robot-assisted dual-extrusion system to conduct the finally printing test. The format of output for motion control of the robot is

\begin{itemize}
    \item xx yy zz nx ny nz e travel\_Flag.
\end{itemize}
The info of each command could be separated as waypoint position (xx yy zz), orientation(nx ny nz) and extrusion volume (e) and travel flag which is used to indicate long-distance travel when new layers or segments start.

We have tested our system by calculating and printing a variety of models with slimmed support structures. Fig.~\ref{fig:sys_pipeline} has shown the whole process of tree support generation for the model Dome, in specifically, the middle part of the Dome is well supported and the support is slimmed as a tree shape. Fig.~\ref{fig:branch_tracing} and Fig.~\ref{fig:implicit_surface} illustrated the tree skeleton and the implicit surface generated based on it. More experimental test is conducted to verify the tree-support generation method in Fig.~\ref{fig:experiments}. Statistic of computation and fabrication is given in Table \ref{tab:compute_and_physical_statistic}.  

\begin{figure}[t]
\includegraphics[width=\linewidth]{fig/printing_result.jpg}
\caption{Examples that are fabricated by our robot system -- (left) Topo-Opt, (middle) Dome and (right) Yoga with supporting structure.}
\label{fig:experiments}
\end{figure}

\begin{table}[t]
\caption{Statistics of compute and physical fabrication.}\vspace{-5pt}
\centering\label{tab:compute_and_physical_statistic}
\footnotesize
\begin{tabular}{r||c|c|c|c|r }
\hline
&\multicolumn{3}{c|}{Compute (sec.)} & \multicolumn{2}{c}{Fabrication}\\
\cline{2-6}
Model   &  Tree Gene. & Boolean & Toolpath & Layer \#  & Time         \\
\hline \hline
Topo-Opt   &  $63.5$ &  $533.1$  &  $63.8$  & $100/137$  &  $13.6$h   \\
Yoga       &  $40.1$ &  $296.5$  &  $10.4$  & $160/177$  &  $10.9$h   \\
Dome       &  $12.5$ &  $79.3 $  &  $4.8$   & $80/92$    &  $3.5 $h   \\
Bridge     &  $52.1$ &  $668.8$  &  $15.4$  & $150/166$  &  $xx.x$h   \\
\hline
\end{tabular}
\end{table}

==> text/system.tex <==
\section{Robotic-assisted 3D printing system}\label{secSystem}
We present a solution for tree support generation for curved layer printing by using a robotic-assisted platform. The overview of our system is illustrated below.

\subsection{Hardware setup}
The hardware setup of our system is mainly composed of a UR5e robot arm which is equipped with a 2IN1 extrusion system. There is a Y-shaped structure and the input of it are two kinds of materials like PLA and PVA which is a water-soluble material used to print support. Different filaments enter the nozzle alternately during the printing process. In specifically, the current filament will retreat to the bifurcation point of the Y-shaped mechanism, and the other one will enter the nozzle through the intersection point when conducting the switch of material. There is only one nozzle that serves as output in our system. And also there is a customized cone-like hotend, which is used to decrease the collision possibility. 

The extruder system is directly mounted on the flange of UR5e, as a result, we can fully utilize the precision of the robot itself and the proven calibration method of the tool coordinate system. There is another inverse configuration shown in \cite{Wu_ICRA17} where the printing platform is mounted on the robot arm and the printing head is fixed on the frame. Its advantage is the high extensibility which could mount different end-effectors like spindle, printing head or probe. But complex calibration work is needed to get a similar result as the counterpart configure we used. And it is not suitable for large volume printing as, with the accumulation of models on the platform, its mass may exceed the load capacity of the robot, and at the same time, it will adversely affect the motion accuracy of the robot. Large pallet inclination will cause the model to fall when the bonding between the model and the pallet is not strong enough. While our setup simplifies the calibration step and is within higher precision, which has better application prospects.

\subsection{Software method}

The main target is to generate a tree-support structure to complete the support generation part of curved layer printing. The basic idea of our work is to trace a tree from branch to trunk, the branch is used to support the overhang regions and the trunk is formed by shrinking the branches together and used to decrease the support usage and printing time. In specifically, a 3D model is sliced into curved layers under different fabrication requirements, an enlarged convex hull will be used to envelop the model, and then model slices and compatible support layers are generated in this envelop mesh. Tree nodes start from the vertices of support-needed faces and then fall from the previous layer to the next layer iteratively, at the same time, aggregate together gradually, which is an inverse process of branching. Then tree-skeleton formed from the previous step could be used to generate a convolution surface to trim the large compatible layers and get the final tree support layer set. The definition of "compatible layers" and "convolution surface" will be explained in Sec.\ref{secAlgorithm}. To the best of our knowledge, this is the first approach to conduct tree support for curved layer printing. See Fig.\ref{fig:sys_pipeline} for an illustration of the pipeline. 

The low-lever software components for controlling the operation of our system are based on the RoboDK. A Duet3D control board is used to supervise the temperature of the nozzle, drive the extrusion motor to feed materials and control the fans. The controller of UR5e, Duet3D board and laptop running RoboDK are linked with each other by the router. The laptop dispatches the motion command and extrusion command to the robot and extruder simultaneously. 
%\tianyu{structure of the robot system}
